Unlocking Spatial Comprehension in Text-to-Image Diffusion Models

We propose CompFuser, an image generation pipeline that enhances spatial comprehension and attribute assignment in text-to-image generative models. Our pipeline enables the interpretation of instructions defining spatial relationships between objects in a scene, such as `An image of a gray cat on the left of an orange dog', and generate corresponding images. This is especially important in order to provide more control to the user. CompFuser overcomes the limitation of existing text-to-image diffusion models by decoding the generation of multiple objects into iterative steps: first generating a single object and then editing the image by placing additional objects in their designated positions. To create training data for spatial comprehension and attribute assignment we introduce a synthetic data generation process, that leverages a frozen large language model and a frozen layout-based diffusion model for object placement. We compare our approach to strong baselines and show that our model outperforms state-of-the-art image generation models in spatial comprehension and attribute assignment, despite being 3x to 5x smaller in parameters.

==> figs/figure4.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0.4cm 0 0 0},clip, width=\linewidth]{images/figure4.pdf}
    \caption{\ours is primarily a conditional text-and-image to image generative model by design. In this figure, we show that this architecture also has the flexibility to be adapted into a conditional text to image model. Note that LDM refers to LLM-grounded diffusion \cite{li2023gligen}.}
    \label{fig:t2i_pipeline}
\end{figure}

==> tables/setup.tex <==
\begin{table}
\centering
\resizebox{0.65\linewidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{$\epsilon$} & \textbf{$c_T$} & \textbf{$c_I$} \\
\midrule
GLIDE \cite{nichol2022glide}                                   & \cmark & \cmark & \xmark  \\
GLIDE + CDM \cite{liu2022compositional}                             & \cmark & \cmark & \xmark  \\
DALL-E mini \cite{Dayma_DALL·E_Mini_2021}                              & \cmark & \cmark & \xmark  \\
CogView2 \cite{ding2022cogview2}                                & \cmark & \cmark & \xmark  \\
InstructPix2Pix\textsuperscript{\dag} \cite{brooks2023instructpix2pix}                         & \cmark & \cmark & \cmark  \\
SD1.5 \cite{Rombach_2022_CVPR}                    & \cmark & \cmark & \cmark  \\
SDXL \cite{podell2023sdxl}                     & \cmark & \cmark & \cmark  \\
\rowcolor{palered}InstructObject2Scene  & \cmark & \cmark & \cmark  \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Input instructions}. $\epsilon$ denotes input noise, $c_T$ represents text instructions, and $c_I$ indicates image instructions. \textsuperscript{\dag}Note that InstructPix2Pix uniquely requires both text and image instructions for generating image.}

\label{tab:setup}
\end{table}
